Risk-averse controller design against data injection attacks on actuators for uncertain control systems

In this paper, we consider the optimal controller design problem against data injection attacks on actuators for an uncertain control system. We consider attacks that aim at maximizing the attack impact while remaining stealthy in the finite horizon. To this end, we use the Conditional Value-at-Risk to characterize the risk associated with the impact of attacks. The worst-case attack impact is characterized using the recently proposed output-to-output $\ell_2$-gain (OOG). We formulate the design problem and observe that it is non-convex and hard to solve. Using the framework of scenario-based optimization and a convex proxy for the OOG, we propose a convex optimization problem that approximately solves the design problem with probabilistic certificates. Finally, we illustrate the results through a numerical example.

==> 7_OOG.tex <==
Let us consider the impact metric used by the system operator is the OOG. Then, similar to \eqref{eqq4}, the adversary with complete system knowledge can obtain for the optimal attack strategy by solving \eqref{g1}
\begin{equation}\label{g1}
\begin{aligned}
q_{OOG}(K,\delta)_{\infty}^2  \triangleq \sup_{a\in \ell_{2e}} \; & \Vert x_p(K,\delta) \Vert_{2}^2 \\
\textrm{s.t.} \quad & \Vert y_r(K,\delta) \Vert_{2}^2 \leq 1, \\
& x(K,\delta)[0]=0,
\end{aligned}
\end{equation}
where $y_r[k]$ is the residual signal for attack detection at time instant $k$, and has the dynamics $y_r[k+1] \triangleq (A-L)y_r[k]$. 

From the system operator's point of view, the best option is to choose a state feedback policy such that the risk of having a huge impact is minimized. This problem can be formulated as:
\begin{problem}\label{problem_2}
Find an optimal state feedback controller $K^*$ such that:
\begin{equation}
K^* = \arg\inf_{K} \text{CVaR}_{\alpha}(q_{OOG}(K,\delta)_{\infty}^2)
\end{equation}
where $\mathcal{R}$ is a measure of risk chosen by the defender. $\hfill\triangleleft$
\end{problem}

As mentioned before, optimizing over a risk metric is difficult since the uncertainty set of the risk metric is continuous. To this end, we can use the steps described in \textit{Section \ref{sec_sample}} to reformulate the risk metric to an empirical risk metric. The reformulation does not differ, except that, we now use the variable $q_{OOG}(\cdot)$ instead of $q(\cdot)$. 

Whilst reformulating, we assume that the impact metric is convex in the design varibale $K$. We showed in \textbf{Section \ref{sec_convex}} that this assumption can be satisfying by using a convex upper bound of $q(\cdot)$. We can similarly show that the metric is in the variable $K$ convex when using OOG. We begin by defining the stacked vectors $\textbf{a}$, and $\textbf{x}$ as defined in \textbf{Section \ref{sec_convex}}. Let us additionally define $\textbf{y}_r \triangleq \begin{bmatrix} y_{r}[0] & \dots & y_r[N_h] \end{bmatrix} $. Here, only the vector $\textbf{a}$ and $\textbf{x}$ are functions of $K$ and $\delta_i$ but they are not explicitly represented as functions, for sake of clarity. The state and the residual stacked vectors are related to the attack vector as $\textbf{x} = F_p(K,\delta_j)\textbf{a}$, and $\textbf{y}_r = F_r(K,\delta_j)\textbf{a}$. Then, $q_{OOG}(K,\delta_i)$ can be reformulated as the non-convex optimization problem \eqref{e1}
\begin{equation}\label{e1}
\begin{aligned}
q_{OOG}(K,\delta_i)_{\infty}^2  \triangleq \sup_{a\in \ell_{2e}} \; & \Vert F_p(K,\delta_j) \textbf{a}\Vert \\
\textrm{s.t.} \quad &  \Vert F_r(K,\delta_j) \textbf{a}\Vert  \leq 1, \\
& x(K,\delta)[0]=0,
\end{aligned}
\end{equation}
The convex dual problem of \eqref{e1} can be formulated as \eqref{e2}. And it was shown in \cite{cdc2021} that the duality gap is zero.
\begin{equation}\label{e2}
\begin{aligned}
\sup_{a\in \ell_{2e}} \; & \gamma \\
\textrm{s.t.} \quad &  F_p^T(\cdot)F_p(\cdot) - \gamma F_r^T(\cdot)F_r(\cdot) \preceq 0.
\end{aligned}
\end{equation}
Pre-multiplying the constraint of \eqref{e2} by $F_r^{-T}(\cdot)$ and post-multiplying by  $F_r^{-1}(\cdot)$, \eqref{e2} can be rewritten as \eqref{e3}.
\begin{equation}\label{e3}
\begin{aligned}
\sup_{a\in \ell_{2e}} \; & \gamma \\
\textrm{s.t.} \quad & (F_p(\cdot)F_r^{-1}(\cdot))^{T}(F_p(\cdot)F_r^{-1}(\cdot))  \preceq \gamma I
\end{aligned}
\end{equation}
And by using the definition of singular values, \eqref{e3} can be re-written as \eqref{e4}.
\begin{equation}\label{e4}
\sup_{a\in \ell_{2e}} \; \sigma_{max} (\underbrace{F_p(\cdot)F_r^{-1}(\cdot)}_{\kappa}) 
\end{equation}

% \clearpage

% \begin{align}
% q_{OOG}(K,\delta)_{\infty}^2 &\triangleq \sup_{a\in \ell_{2e}} \;  \frac{\Vert x_p(K,\delta) \Vert_2^2}{\Vert y_r(K,\delta) \Vert_2^2} \\
% &= \sup_{\textbf{a}} \frac{\Vert F_p(K,\delta_j)\textbf{a} \Vert_2^2}{\Vert F_r(K,\delta_j)\textbf{a} \Vert_2^2}\\
% &\leq_{2} \sup_{\textbf{a}} \frac{\Vert F_p(K,\delta_j) \Vert_2^2\Vert \textbf{a} \Vert_2^2}{\Vert F_r(K,\delta_j)\Vert_2^2\Vert \textbf{a}\Vert_2^2}\\
% &= \frac{\Vert F_p(K,\delta_j) \Vert_2^2}{\Vert F_r(K,\delta_j)\Vert_2^2}\\
% &= \Vert F_p(K,\delta_j) \Vert_2^2(\Vert F_r(K,\delta_j)\Vert_2^2)^{-1} \label{g2}
% \end{align}
% where the inequality $2$ follows since the matrix $2$ norm is a sub-ordinate norm.

% We known that matrix norm obeys the inequality $(||A||)^{-1} \leq ||A^{-1}||$. So we can reformulate \eqref{g2} as 
% \begin{equation}\label{g3}
% q_{OOG}(K,\delta)_{\infty}^2 \leq \Vert F_p(K,\delta_j) \Vert_2^2\Vert F_r^{-1}(K,\delta_j)\Vert_2^2.
% \end{equation}
% The matrix norm obeys the inequality $||AB|| \leq ||A||||B||$. So we can reformulate \eqref{g3} as
% \begin{align}
% q_{OOG}(K,\delta)_{\infty}^2 & \geq\mathord{?}\leq \Vert \underbrace{F_p(K,\delta_j) F_r^{-1}(K,\delta_j)}_{\kappa}\Vert_2^2 \label{g4},\\
% &= \sigma_{max}(\kappa)
% \end{align}
% In \eqref{g4}, we cannot be sure if the inequality is $\geq$ or $\leq$. This is because $\kappa$ is a lower bound to the term $\Vert F_p(K,\delta_j) \Vert_2^2\Vert F_r^{-1}(K,\delta_j)\Vert_2^2$. \textbf{This point is the main limitation and should be discussed before we proceed with this idea. }

Next we proceed to show that $\sigma_{max}(\kappa)$ is convex in the the design variable $K$. To this end, we first rewrite the term in \textit{Lemma \ref{lem_oog_1}}.
\begin{lemma}\label{lem_oog_1}
It holds that
\begin{multline}\label{g6}
\sigma_{max}(\kappa) \leq \det(B(\delta_j))^{N_h-1}\big( \frac{\sum_{i=1}^{nN_h-1}\sigma_i(\kappa^{-1})}{nN_h-1} \big)^{n_uN_h-1}   
\end{multline}
$\hfill\square$
\end{lemma}

The above lemma states that $\sigma_{max}(\kappa)$ can be approximated with a bound which is given on right side of the inequality \eqref{g6}. However, only the term
\begin{equation}\label{g7}
   \bar{q}(K,\delta_j)_{OOG} = \bar{Q}_{j}(K) \triangleq \sum_{i=1}^{nN_h-1}\sigma_i(\kappa^{-1}))
\end{equation}
of the inequality is dependent on the controller variable $K$. Thus, the term $\bar{Q}(K,\delta_j)$ can be replaced as the bound. It remains to show that this term is indeed convex. This is shown in the following lemma:
\begin{lemma}\label{lem_oog_2}
The function $\bar{Q}(K,\delta_j)$ is convex in the variable $K$. $\hfill\square$
\end{lemma}
\begin{proof}
The proof directly follows from \cite[Theorem V.1]{dvijotham2014convex}. However, the outline of the proof is stated here. It can be shown that $F_p(K,\delta_i)^{-1}$ takes the form as in \eqref{matrix_F}. The convexity of $F(K,\delta_i)^{-1}$ is immediate since it is affine in $K$. The matrix $F_{r}(K,\delta_i)^{-1}$ is independent of the design variable $K$ and thus is convex. And therefore the product of the two matrices is linear in the term $K$ and thus convex.

It can be further shown that the function $X \to \sigma(X)$ is convex \cite{lewis1995convex}. Since $\bar{Q}(K,\delta_j)$ is a affine combination of $\sigma(X)$, it is convex which concludes the proof. 
\end{proof}

We have shown in \textit{Lemma \ref{lem_oog_1}} that the term $\bar{Q}(K,\delta_j)$ can be used as an upper/lower bound for $\bar{q}(K,\delta_j)_{OOG}$. We have shown in \textit{Lemma \ref{lem_oog_2}} that this term is convex. Using this convex bound, we recast \textit{Problem 2} as \eqref{g8}.
\begin{equation}\label{g8}
\begin{aligned}
\arg \inf_{K,y} & y\\
\textrm{s.t.} \; & \frac{1}{k}\sum_{j=1}^k\bar{Q}_{i_j}(K)^2 \leq y,\\
&\forall \text{choice of $k$ indices} \{i_1,\dots,i_k\} \subseteq \{1,\dots,N\}
\end{aligned}
\end{equation}

Then, we can use the \textbf{Algorithm \ref{algo1}} to summarize the solution method in our paper. To show the effectiveness of the design approach, we used the same numerical example as described in \textit{Section \ref{sec_NE}}. Let $C_r=C_p=I_3$ and $D_r=D_p=0$. The only difference is that now we use the OOG as an impact metric. We solve \eqref{g8} and obtain the optimal arguments $y_N^*$ as $36.00$ and 
\[
K_N^*=\begin{bmatrix}
   -1.3831  &  2.1178  &  -5.2263\\
    3.3333  &  -2.1178  &   6.2263\\
   -0.0000 &  1.0000  &  -0.8679
\end{bmatrix}.
\]
To recall, $K_N^*$ represents the optimal controller which minimizes the CVaR$_{\alpha}$ for \eqref{problem_2} under data injection attacks. And $y_N^*$ represents the CVaR$_{\alpha}$.
